ValUES: A Framework for Systematic Validation of Uncertainty Estimation in Semantic Segmentation

Uncertainty estimation is an essential and heavily-studied component for the reliable application of semantic segmentation methods. While various studies exist claiming methodological advances on the one hand, and successful application on the other hand, the field is currently hampered by a gap between theory and practice leaving fundamental questions unanswered: Can data-related and model-related uncertainty really be separated in practice? Which components of an uncertainty method are essential for real-world performance? Which uncertainty method works well for which application? In this work, we link this research gap to a lack of systematic and comprehensive evaluation of uncertainty methods. Specifically, we identify three key pitfalls in current literature and present an evaluation framework that bridges the research gap by providing 1) a controlled environment for studying data ambiguities as well as distribution shifts, 2) systematic ablations of relevant method components, and 3) test-beds for the five predominant uncertainty applications: OoD-detection, active learning, failure detection, calibration, and ambiguity modeling. Empirical results on simulated as well as real-world data demonstrate how the proposed framework is able to answer the predominant questions in the field revealing for instance that 1) separation of uncertainty types works on simulated data but does not necessarily translate to real-world data, 2) aggregation of scores is a crucial but currently neglected component of uncertainty methods, 3) While ensembles are performing most robustly across the different downstream tasks and settings, test-time augmentation often constitutes a light-weight alternative. Code is at: https://github.com/IML-DKFZ/values

==> tables/separation_study_summary.tex <==
\begin{table}[t]
    \caption{\textbf{\rebuttal{Findings} of the separation study.} Green denotes agreement with theoretical claims, red indicates contradictions, and orange represents partial agreement or contradiction. \rebuttal{Underlying quantitative results on LIDC and GTA5/CS are provided in \autoref{fig:main_results_barplot} and details, including results on the toy dataset, in \autoref{appendix:separation}}.}
    %\label{tab:separation_study_summary}
    \centering
    \footnotesize
            \renewcommand{\arraystretch}{1.25}
    \resizebox{0.8\linewidth}{!}{
    \begin{tabular}{l|l|c|c|c}
        Question & \shortstack{Qual./Quant.} & Toy Dataset & LIDC & GTA5/CS\\ 
        \cmidrule[1.5pt]{1-5}
        \multirow{2}{*}{Q1: Do AU-measures capture AU?} & Quantitative & {\cellcolor[HTML]{93c47d} yes} & {\cellcolor[HTML]{f6b26b} partially} & {\cellcolor[HTML]{f6b26b} partially}\\
        \cline{2-5}
         & Qualitative & {\cellcolor[HTML]{93c47d} yes} & {\cellcolor[HTML]{f6b26b} often (i.i.d.)} & {\cellcolor[HTML]{f6b26b} partially}\\
        \cline{1-5}
        \multirow{2}{*}{Q2: Do EU-measures capture AU?} & Quantitative & {\cellcolor[HTML]{93c47d} no} & {\cellcolor[HTML]{e06666} often yes} & {\cellcolor[HTML]{93c47d} no}\\
        \cline{2-5}
         & Qualitative & {\cellcolor[HTML]{93c47d} no} & {\cellcolor[HTML]{e06666} often yes} & {\cellcolor[HTML]{93c47d} no}\\
        \cmidrule[1.5pt]{1-5}
        Q3: Do EU-measures capture EU? & Quantitative & {\cellcolor[HTML]{93c47d} yes} & {\cellcolor[HTML]{93c47d} yes} & {\cellcolor[HTML]{93c47d} yes}\\
        \cline{1-5}
        Q4: Do AU-measures capture EU? & Quantitative & {\cellcolor[HTML]{f6b26b} depends on  AU in data} & {\cellcolor[HTML]{f6b26b} partially no} & {\cellcolor[HTML]{93c47d} mostly not}\\
    \end{tabular}
    }
\end{table}

==> tables/thresholds_unc_aggregation.tex <==
\begin{table}[h!]
\scriptsize
\centering
\caption{Thresholds for the uncertainty aggregation obtained with \autoref{eq:threshold}. The rows show the different prediction models and the columns the thresholds for the different uncertainty types.}
\begin{tabular}{p{2cm}||p{2cm}|p{2cm}|p{2cm}}
\toprule
 & \bfseries Epistemic & \bfseries Aleatoric & \bfseries Predictive \\
\midrule
\midrule
\bfseries Deterministic & - & - & $8.6242e-06$ \\
\cmidrule{1-4}
\bfseries TTD & $0.0002652523$ & $0.0011531989$ & $0.0015468701$ \\
\cmidrule{1-4}
\bfseries Ensemble & $4.82736e-05$ & $0.0004489746$ & $0.0005115819$ \\
\cmidrule{1-4}
\bfseries SSN & $0.024855889$ & $0.0047146515$ & $0.0307405433$ \\
\bottomrule
\end{tabular}
\label{tab:thresholds_unc_aggregation}
\end{table}
